Adaptive Image Denoising by Mixture Adaptation

We propose an adaptive learning procedure to learn patch-based image priors for image denoising. The new algorithm, called the Expectation-Maximization (EM) adaptation, takes a generic prior learned from a generic external database and adapts it to the noisy image to generate a specific prior. Different from existing methods that combine internal and external statistics in ad-hoc ways, the proposed algorithm is rigorously derived from a Bayesian hyper-prior perspective. There are two contributions of this paper: First, we provide full derivation of the EM adaptation algorithm and demonstrate methods to improve the computational complexity. Second, in the absence of the latent clean image, we show how EM adaptation can be modified based on pre-filtering. Experimental results show that the proposed adaptation algorithm yields consistently better denoising results than the one without adaptation and is superior to several state-of-the-art algorithms.

==> parameter_tuning.tex <==
\section{Choice of Parameters}
\label{section4}

In this section, we discuss the choice of some parameters, including those in EPLL denoising and those in GMM adaptation. 

\subsection{Parameters in EPLL Denoising}
In EPLL, the parameter $\gamma$ plays an important role in solving the subproblems \eref{subproblem: solve for v_i} and \eref{subproblem: solve for x}. The choice of $\gamma$ is an open question. Typically, $\gamma$ is inverse proportional to the amount of noise present in the image patch $\mP_i\vx$. At iteration 1 when we initialize $\vx$ with the noisy image $\vy$, $\gamma$ is set to $\frac{1}{\sigma^2}$, while as the iteration continues, $\vx$ is replaced by some cleaner estimate $\hat{\vx}$, thus the value of $\gamma$ increases. EPLL empirically sets $\gamma = \frac{1}{\sigma^2}(1, 4, 8, 16, 32)$ and demonstrates its good performance experimentally. 

Besides the explicit parameter $\gamma$, EPLL has another implicit parameter. Note that in \eref{GMM-MAP:x} we use $\mP_i\vx$ to compute the posterior probabilities and then find a cluster for each patch. However, in practice we have no access to the ground truth $\vx$. We thus have to replace $\vx$ with $\vy$ or some estimate $\hat{\vx}$. In consequence \eref{GMM-MAP:x} also needs to be modified.
\begin{equation}
\argmax{i} \;\frac{\vpi_i \calN(\mP_i\hat{\vx}| \vmu_i, \mSigma_i + \delta\mI)}{\sum_{l = 1}^{k} \vpi_l \calN(\mP_i\hat{\vx}| \vmu_l, \mSigma_l + \delta\mI)}.
\label{GMM-MAP:xhat}
\end{equation} 
Unlike $\gamma$, $\delta$ is proportional to the amount of noise in the image $\hat{\vx}$, and is thus set to be $\sigma^2(1, \frac{1}{4}, \frac{1}{8}, \frac{1}{16}, \frac{1}{32})$. 

\subsection{Parameters in GMM Adaptation}
The performance of EPLL greatly depends on the quality of the prior distribution, \emph{i.e.}, the learned GMM. The current GMM employed by EPLL is learned from a large generic database and is thus termed a $generic$ or $universal$ prior model. In other words, no prior information about the image of interest is utilized when learning the GMM. We have introduced GMM adaptation in Section II-B. In this subsection, we discuss its important parameters in the implementation. 

Recall that GMM adaptation consists of two steps where the E-step computes the posterior probabilities in \eref{posterior probabilities} while the M-step performs adaptation in \eref{weight adaptation}, \eref{mean adaptation} and \eref{covariance adaptation} (or \eref{simplified covariance adaptation}) by combining the old and new parameters. 

Equation \eref{posterior probabilities} computes the posterior probabilities for patches $\vp_1,\ldots,\vp_n$. Ideally, these patches should be from the clean image $\vx$. However, in reality we only have the \emph{perturbed} patches, for example, the noisy observations $\vq_1,\ldots,\vq_n$ or the denoised patches $\hat{\vp}_1,\ldots,\hat{\vp}_n$. Letting the perturbed patches as $\vq_i^{\vepsilon_i} = \vp_i + \vepsilon_i$ with $\vepsilon_i$ being the perturbation, we assume for simplicity that $\vepsilon_i \sim \calN(\vzero, \tilde{\sigma}^2\mI)$.  We then revise 

In our experiments, we find empirically that for noisy observations $\vq_1,\ldots,\vq_n$, $\vepsilon_i = \sigma^2$ (the noise variance) works best, while for the denoised patches $\hat{\vp}_1,\ldots,\hat{\vp}_n$ (results from the original EPLL denoising), $\vepsilon_i = (0.25\sigma)^2$ to $(0.35\sigma)^2$ can achieve similar best denoising performance.  

The other important parameter in GMM adaptation is the relevance factor $\rho$ in \eref{adaptation coefficient}. This is because $\rho$ controls the adaptation coefficient $\alpha_i$, and thus determines how much the weights, means and covariances are adapted in \eref{weight adaptation}, \eref{mean adaptation} and \eref{covariance adaptation} (or \eref{simplified covariance adaptation}). Intuitively, the choice of $\rho$ relies on our belief in the new patches for adaptation. If the new patches are trustworthy such as the relevant clean patches, we should choose a small $\rho$ to adapt more. On the contrary, if the new patches are less trustworthy such as the noisy patches, we should choose a large $\rho$ to adapt less. We conduct experiments to show how different $\rho$s affect the denoising performance in two cases. In Figure \ref{fig:rho effect} (a), we consider the $\rho$ effect when a noisy image is used for GMM adaptation. As we can see, a large $\rho$ yields a higher PSNR value than a small $\rho$, indicating that since the image for adaptation is noisy, we should choose a large $\rho$ to adapt less. In Figure \ref{fig:rho effect} (b), we consider the $\rho$ effect when a ground-truth clean image is used for GMM adaptation. Different from (a), the plotted curves show that a small $\rho$ outperforms a large $\rho$. This result is consistent with our belief that since the patches for adaptation are reliable clean patches, we should choose a small $\rho$ to adapt more. 

\begin{figure}[h]
\centering
\def\iw{0.47\linewidth}
\begin{tabular}{cc}
\includegraphics[width=\iw]{/rho_effect/rho_effect_on_noisy_inputs.eps}&
\includegraphics[width=\iw]{/rho_effect/rho_effect_on_clean_inputs.eps}\\
(a) \scriptsize{noisy image for adaptation} & (b) \scriptsize{clean image for adaptation} \\
\end{tabular}
\caption{Test images of size 128 $\times$ 128}
\label{fig:rho effect}
\end{figure}



